Trapped and Unstable: Axion-like particle fragmentation at finite temperature

We investigate the emergence of a resonant behavior in axion-trapped misalignment models featuring finite-temperature potential barriers. As the temperature decreases and the field is released from its trapped configuration, inhomogeneities are exponentially amplified through an instability in their equation of motion, leading to the fragmentation of the axion field. We show that this process constitutes a novel source of gravitational waves (GWs), analogous to those generated in zero-temperature axion fragmentation, but with distinct characteristics. We quantify the resulting GW spectrum, identifying the peak frequency and amplitude associated with the inhomogeneous axion dynamics. Our results indicate that the GW signal can be enhanced by up to two orders of magnitude compared to the standard fragmentation scenario, while exhibiting a markedly different spectral shape. The parameter space featuring both strong GW signals and reproducing the correct dark matter abundance is, however, limited.

==> preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{hyperref}
\usepackage{array}
\usepackage{soul}
\usepackage{xcolor}
\usepackage{comment}
\usepackage{physics}
\usepackage{cancel}
\usepackage{slashed}

\widowpenalty=500
\clubpenalty=500
\enlargethispage{\baselineskip}
\usepackage{orcidlink}
\usepackage{csquotes}
\hypersetup{
     colorlinks   = true,
     citecolor    = black,
     breaklinks = true,
     urlcolor = black,
     linkcolor = black
}

% ==================================================================================================
%  Inserting some useful commands
% ==================================================================================================
\newcommand{\Appendix}{Appendix}


\newcommand{\de}{\mathrm{d}}
\newcommand{\GeV}{\,\mathrm{GeV}}
\newcommand{\MeV}{\,\mathrm{MeV}}


%%%%%%%%%%%%%%% macros %%%%%%%%%%%%%%%
\renewcommand{\vec}[1]{{\bf #1}}
\newcommand{\rmi}[1]{{\mbox{\scriptsize #1}}}
\newcommand{\rmii}[1]{{\mbox{\tiny\rm{#1}}}}
\newcommand{\nn}{\nonumber \\}



\newcommand{\Mpl}{M_\rmii{Pl}}


